Laser-induced Creation of antiferromagnetic 180-degree domains in NiO/Pt bilayers

We demonstrate how the antiferromagnetic order in heterostructures of NiO/Pt thin films can be modified by optical pulses. We irradiate our samples with laser light and identify an optically induced creation of antiferromagnetic domains by imaging the created domain structure utilizing the X-ray magnetic linear dichroism effect. We study the effect of different laser polarizations on the domain formation and identify a polarization-independent creation of 180{\deg} domain walls and domains with 180{\deg} different N\'eel vector orientation. By varying the irradiation parameters, we determine the switching mechanism to be thermally induced and demonstrate the reversibility. We thus demonstrate experimentally the possibility to optically create antiferromagnetic domains, an important step towards future functionalization of all optical switching mechanisms in antiferromagnets.

==> name.tex <==

\author{Andrew N. Other}
\altaffiliation{A shared footnote}
\author{Fred T. Secondauthor}
\altaffiliation{Current address: Some other place, Othert\"own,
Germany}
\author{I. Ken Groupleader}
\altaffiliation{A shared footnote}
\email{i.k.groupleader@unknown.uu}
\phone{+123 (0)123 4445556}
\fax{+123 (0)123 4445557}
\affiliation[Unknown University]
{Department of Chemistry, Unknown University, Unknown Town}
\alsoaffiliation[Second University]
{Department of Chemistry, Second University, Nearby Town}
\author{Susanne K. Laborator}
\email{s.k.laborator@bigpharma.co}
\affiliation[BigPharma]
{Lead Discovery, BigPharma, Big Town, USA}
\author{Kay T. Finally}
\affiliation[Unknown University]
{Department of Chemistry, Unknown University, Unknown Town}
\alsoaffiliation[Second University]
{Department of Chemistry, Second University, Nearby Town}


